Trace estimates for harmonic functions along circular arcs with applications to domain decomposition on overlapping disks

In this paper we derive several (and in many cases sharp) estimates for the $\mathrm{L}^2$-trace norm of harmonic functions along circular arcs. More precisely, we obtain geometry-dependent estimates on the norm, spectral radius, and numerical range of the Dirchlet-to-Dirichlet (DtD) operator sending data on the boundary of the disk to the restriction of its harmonic extension along circular arcs inside the disk. The estimates we derive here have applications in the convergence analysis of the Schwarz domain decomposition method for overlapping disks in two dimensions. In particular, they allow us to establish a rigorous convergence proof for the discrete parallel Schwarz method applied to the Conductor-like Screening Model (COSMO) from theoretical chemistry in the two-disk case, and to derive error estimates with respect to the discretization parameter, the number of Schwarz iterations, and the geometry of the domain. Our analysis addresses challenges beyond classical domain decomposition theory, especially the weak enforcement of boundary conditions.

==> bipolarSection.tex <==
\section{An $\mL^2$-maximum principle on the infinite strip}\label{sec:2}

As stated in the introduction, the goal of this section is to first reformulate the $\mL^2$ estimates for circular arcs across the disk in Theorem~\ref{thm:main} as weighted $\mL^2$ estimates for horizontal straight lines on the infinite horizontal strip 
\begin{align}
	\mathcal{S} \coloneqq \R \times (0,2\pi). 
\end{align}

To do so, we will make use of the well-known bipolar transform, whose definition and main properties we recall below. Additionally, we will recall a few properties of the Poisson kernel on the infinite strip, which will be a key technical tool in our proof of the sought-after weighted $\mL^2$ estimates on the infinite strip. %Finally, we will compute the Fourier transform of the Poisson kernel on the infinite strip and prove certain technical lemmas that will be used in the subsequent Section~\ref{sec:mainproofs} to complete our proof of Theorem~\ref{thm:main}. 
Throughout this section, we will assume the setting and notation introduced in Section \ref{sec:1}. 

\subsection{The bipolar transform}

Let $\Omega \subset \R^2$ be an open disk and let $\Gamma \subset \Omega$ be a circular arc across $\Omega$ in the sense of Definition \ref{def:notation}. The starting point of our analysis is the observation that the sought-after Estimates~\eqref{eq:New_1_int} and~\eqref{eq:New_1_ext}  %from Theorem \ref{thm:main} 
are invariant under translations, rotations, and dilations of the chosen coordinate system. Therefore, we can assume without loss of generality that the intersection points $\{\mathbf{a}_1, \mathbf{a}_2\} = \partial \Omega \cap \overline{\Gamma}$ are given by
\begin{align*}
	\mathbf{a}_1 := (-1, 0)\quad \mbox{and}\quad \quad \mathbf{a}_2 := (1, 0),
\end{align*}
and that $\Gamma$ is located on the lower half-plane $\{ (x,y) \in \R^2 : y\leq 0 \}$. An example of this geometric setting is displayed in Figure \ref{fig:01a}. 



\begin{figure}[h!]
	\centering
	\begin{subfigure}{0.48\textwidth}
		\centering
		\input{geometric_setting.tex}
		\caption{ }		
		\label{fig:01a}
	\end{subfigure}\hfill
	\begin{subfigure}{0.48\textwidth}
		\centering
		\input{constant_curves.tex}
		\caption{ }
		\label{fig:01b}
	\end{subfigure}
        \caption{(a) An example of the geometric setting and (b) curves of constant $\sigma$ in Cartesian space.}
	\label{fig:01}
\end{figure}


  Based on this observation, we introduce the so-called bipolar coordinate system with poles (or foci) at $\{\mathbf{a}_1, \mathbf{a}_2\}:=\{(-1,0),(1,0)\}$. 



\begin{definition}[Bipolar Transform]\label{def:Bipolar} Let $\mathcal{S} = \R \times (0,2\pi) \subset \mathbb{R}^2$ denote the infinite horizontal strip. We define the bipolar transform as the mapping $\Psi \colon \mathcal{S} \rightarrow \mathbb{R}^2$ given by
	\begin{align}
		\Psi(\tau, \sigma) :=\left( \frac{\sinh(\tau)}{\cosh(\tau)-\cos(\sigma)}, \frac{-\sin(\sigma)}{\cosh(\tau)-\cos(\sigma)}\right) \qquad \forall (\tau, \sigma) \in \mathcal{S}. \label{eq:bipolardef}
	\end{align}
	\end{definition}




The bipolar transform has a number of useful properties that can, for instance, be found in \cite{MorseFeshbach53}. We list two in particular that will be crucial for our subsequent analysis. 

\begin{proposition}[The bipolar transform]\label{prop:bipolartransform} The bipolar transform $\Psi \colon \mathcal{S} \rightarrow \mathbb{R}^2$ defined through Definition \ref{def:Bipolar} has the following properties:
\begin{enumerate}[label=(\roman*)]
\item $\Psi$ is a conformal\footnote{In the sense that the Jacobian $\mD \Psi (\tau, \sigma)$ at any $(\tau, \sigma) \in \mathcal{S}=\R^2 \times (0, 2\pi)$ is the product of a non-zero (not necessarily positive) scalar and an orthogonal matrix.} diffeomorphism from the strip $\mathcal{S}$ to the set $\mathbb{R}^2 \setminus \left\{ (x,0) \in \R^2 : |x| \geq 1 \right\}$. 
	
\item \label{it:disks} For any $\sigma\in (0, \pi)$, the bipolar transform $\Psi$ maps the open strip $\mathcal{S}_\sigma = \R \times (\sigma,\sigma+\pi)$ to the open disk $\Psi(\mathcal{S}_\sigma) = \Omega \subset \R^2$ such that $\{\mathbf{a_1},\mathbf{a_2}\} \subset \partial \Omega$. Moreover, the lines $\R_\sigma = \R \times \{\sigma\}$ and $\R_{\sigma+\pi}= \R \times \{\sigma+\pi\}$ are mapped to the portions of the boundary $\partial \Omega$ in the lower and upper half-plane, respectively, i.e.,
\begin{align*}
		\partial \Omega = \underbrace{\{(x, y) \in \partial \Omega \colon y < 0\}}_{=\Psi(\mathbb{R}_\sigma)} \cup \underbrace{\{(x, y) \in \partial \Omega \colon y >0\}}_{= \Psi(\mathbb{R}_{\sigma+\pi})} \cup \{\mathbf{a}_1, \mathbf{a}_2\}.
	\quad \mbox{
	(See Figure~\ref{fig:01b}.)} \end{align*}
Conversely, for any open disk $\Omega \subset \R^2$ satisfying $\{\mathbf{a}_1, \mathbf{a}_2 \}\subset \partial\Omega$ there exists $\sigma \in (0,\pi)$ such that $\Omega = \Psi(\mathcal{S}_\sigma)$.
	\end{enumerate}

 
\end{proposition}

  In view of Property~\ref{it:disks} of Proposition~\ref{prop:bipolartransform}, we introduce the following weighted Lebesgue spaces.

\begin{definition}[Weighted Lebesgue Spaces]\label{def:Leb_w} Let $\Psi \colon \mathcal{S} \rightarrow \mathbb{R}^2$ be the bipolar transform introduced in Definition~\ref{def:Bipolar}, let $\sigma \in (0,2\pi)$, let $p\in [1,\infty]$, and let $\Psi_{\sigma} \colon \R_\sigma \rightarrow \Psi(\R_\sigma)$ be the restriction $\Psi_\sigma = \Psi \rvert_{\R_{\sigma}}$ where $\R_\sigma := \R \times \{\sigma\}$. Then we define the weighted Lebesgue space $\mathcal{L}^p_{\sigma}$ as the vector space 
	\begin{align*}
		\mathcal{L}^p_{\sigma}	:=\{f \colon \mathbb{R}_{\sigma}\rightarrow \mathbb{C} ~\text{ such that } f\circ \Psi_{\sigma}^{-1}\in \mL^p(\Psi(\mathbb{R}_{\sigma}))\},
	\end{align*}
	endowed with the norm $\Vert f \Vert_{\mathcal{L}^p_{\sigma}} :=\Vert f  \circ \Psi^{-1} \Vert_{\mL^p(\Psi(\mathbb{R}_{\sigma}))}$, where $\mL^p\bigr(\Psi(\R_\sigma)\bigr)$ denotes the $\mL^p$ space with respect to the one-dimensional Hausdorff measure on the circular arc $\Psi(\R_\sigma)$. 
\end{definition}

\begin{remark}[Alternative definition]\label{def:Leb_w_2} From the change of variables formula we can equivalently define $\mathcal{L}^p_\sigma$ as the vector space of (Lebesgue) measurable functions $f:\R \rightarrow \C$ satisfying
\begin{align}
     \Vert f \Vert_{\mathcal{L}^p_{\sigma}}^p  :=  \int_{-\infty} ^{\infty} \vert f(\tau)\vert^p \frac{1}{\cosh(\tau) - \cos(\sigma)}\, d\tau < \infty .\label{eq:weightednorm}
\end{align}
In the sequel, we will frequently make use of this alternative representation of the weighted Lebesgue space $\mathcal{L}^p_{\sigma}$ without further comment.
\end{remark}

\textcolor{orange}{We can now restate the estimates from Theorem~\ref{thm:main} as estimates for harmonic functions in the strip $\mathcal{S} = \R \times (0,2\pi)$.
\begin{lemma}[$\mL^2$-estimates on the infinite strip]\label{lem:L2maxstrip} Let $\Psi\colon \mathcal{S} \rightarrow \R^2$ be the bipolar transform introduced in Definition~\ref{def:Bipolar}, let $\mathcal{L}^2_\sigma$ for $\sigma \in (0,2\pi)$ be the weighted Lebesgue spaces introduced in Definition~\ref{def:Leb_w}, and recall the notation $\mathcal{S}_\sigma \coloneqq \R \times(\sigma,\sigma+\pi)$. Then estimates~\eqref{eq:New_1_int}--\eqref{eq:New_1_full} hold for any open disk $\Omega$ and any circular arc $\Gamma$ across $\Omega$ if and only if the estimates 
\begin{align}
    &\norm{(u_{\Psi^\#h}\circ \Psi)(\cdot, \sigma+\theta)}_{\mathcal{L}^2_{\sigma+\theta}}^2 < \frac{1-\cos(\theta)}{2} \norm{h}_{\mathcal{L}^2_{\sigma+\pi}}^2,  \label{eq:New_2_int} 
    \\[0.5em]
	&\norm{(u_{\Psi^\#g}\circ \Psi) (\cdot, \sigma+\theta)}_{\mathcal{L}^2_{\sigma+\theta}}^2 < \frac{1+\cos(\theta)}{2} \norm{g}_{\mathcal{L}^2_{\sigma}}^2,  \label{eq:New_2_ext} \\[0.5em]
&\norm{\big((u_{\Psi^\#g}+u_{\Psi^\#h})\circ \Psi\big)(\cdot, \sigma+\theta)}_{\mathcal{L}^2_{\sigma+\theta}}^2 < \norm{g}_{\mathcal{L}^2_{\sigma}}^2+\norm{h}_{\mathcal{L}^2_{\sigma+\pi}}^2, \label{eq:New_2_full}
\end{align}
hold for any $g\in \mathcal{L}^2_\sigma, h\in \mathcal{L}^2_{\sigma+\pi}$ and for any $\theta,\sigma \in (0,\pi)$, where $u_{\Psi^\#g}$ and $u_{\Psi^\#h}$ are the Poisson integrals of $\Psi^\# g$ and $\Psi^\#h$ in the disk $\Psi(\mathcal{S}_\sigma)$, i.e., 
\begin{align*}
    u_{\Psi^\# g}(\mathbf{x})& \coloneqq \frac{1}{2\pi} \int_{\Psi(\R_\sigma)} \frac{r_\sigma^2 -|\mathbf{x}-\mathbf{x_\sigma}|^2}{r_\sigma |\mathbf{x}-\mathbf{y}|^2} (g\circ \Psi^{-1})(\mathbf{y}) \mathrm{d} \mathcal{H}^1(\mathbf{y}), \quad \mathbf{x} \in \Psi(\mathcal{S}_\sigma),\\
    u_{\Psi^\# h}(\mathbf{x}) &\coloneqq \frac{1}{2\pi} \int_{\Psi(\R_{\sigma+\pi})} \frac{r_\sigma^2 -|\mathbf{x}-\mathbf{x_\sigma}|^2}{r_\sigma |\mathbf{x}-\mathbf{y}|^2} (h\circ \Psi^{-1})(\mathbf{y}) \mathrm{d} \mathcal{H}^1(\mathbf{y}), \quad \mathbf{x} \in \Psi(\mathcal{S}_\sigma),
\end{align*}
where $r_\sigma>0$ and $\mathbf{x}_\sigma \in \R^2$ denote respectively the radius and center of the disk $\Psi(\mathcal{S}_\sigma)$. Additionally, %Estimates~\eqref{eq:New_1_int},~\eqref{eq:New_1_ext}
Estimates~\eqref{eq:New_1_int}--\eqref{eq:New_1_full} are sharp if and only if Estimates \eqref{eq:New_2_int}--\eqref{eq:New_2_full} are sharp.
\end{lemma}}


\begin{proof} 

Let $\Gamma$ be a given circular arc across the open disk $\Omega$ and denote by $\theta_{\Gamma}$ the associated angle (see Definition \ref{def:notation}). From the discussion in the beginning of this section, we can assume without loss of generality that $\partial \Omega \cap \overline{\Gamma} = \{(-1,0),(1,0)\}$ and the arc $\Gamma$ lies in the lower half-plane. Hence, by Proposition~\ref{prop:bipolartransform}, there exist $\sigma_\Omega \in (0,\pi)$ and $\sigma_\Gamma \in (0,\pi)$ such that 
\begin{align}
    \Omega = \Psi(\mathcal{S}_{\sigma_\Omega})\quad \mbox{and}\quad \Gamma = \Psi(\R_{\sigma_\Gamma}). \label{eq:sigmaomega0}
\end{align}
Moreover, the angle $\theta_\Gamma$ associated to the arc $\Gamma$ (see also Figure~\ref{fig:01a}) is given by
\begin{align}
	\theta_\Gamma = \sigma_\Gamma - \sigma_\Omega.   \label{eq:thetaid}
\end{align}
Therefore, assuming that Estimates~\eqref{eq:New_2_ext} and \eqref{eq:New_2_int} hold, we immediately deduce from the definition of the weighted Lebesgue spaces $\mathcal{L}^2_\sigma$ that the estimates
\begin{align*}
	&\norm{u_{\Psi^\#g}}_{\mL^2(\Gamma)}^2 = \norm{(u_{\Psi^\#g}\circ \Psi) (\cdot, \sigma_\Omega+\theta_\Gamma)}_{\mathcal{L}^2_{\sigma_\Omega+\theta_\Gamma}}^2 < \frac{1+\cos(\theta_\Gamma)}{2} \norm{g}_{\mathcal{L}^2_{\sigma_\Omega}}^2 = \frac{1+\cos(\theta_\Gamma)}{2} \norm{\Psi^\# g}_{\mL^2(\partial \Omega^{\rm ext})}^2, \\
	&\norm{u_{\Psi^\# h}}_{\mL^2(\Gamma)}^2 = \norm{(u_{\Psi^\# h}\circ \Psi)(\cdot, \sigma_\Omega+\theta_\Gamma) }_{\mathcal{L}^2_{\sigma_\Omega+\theta_\Gamma}}^2 < \frac{1-\cos(\theta_\Gamma)}{2} \norm{h}_{\mathcal{L}^2_{\sigma_\Omega+\pi}}^2 = \frac{1-\cos(\theta_\Gamma)}{2} \norm{\Psi^\# h}_{\mL^2(\partial \Omega^{\rm int})}^2
\end{align*} 
hold for any $g \in \mathcal{L}^2_{\sigma_\Omega}$ and any $h \in \mathcal{L}^2_{\sigma_\Omega+\pi}$. These are precisely Estimates~\eqref{eq:New_1_int} and~\eqref{eq:New_1_ext}.  Thus, since the push-forward maps $g \in \mathcal{L}^2_{\sigma_\Omega} \mapsto g\circ \Psi^{-1} \rvert_{\partial \Omega^{\rm ext}} \in L^2(\partial \Omega^{\rm ext})$ and $h \in \mathcal{L}^2_{\sigma_\Omega+\pi} \mapsto h \circ \Psi^{-1} \rvert_{\partial \Omega^{\rm int}} \in L^2(\partial \Omega^{\rm int})$ are bijective, we conclude that Estimates~\eqref{eq:New_1_int} and \eqref{eq:New_1_ext} holds for any $g \in \mL^2(\partial \Omega^{\rm int})$ and any $h\in \mL^2(\partial \Omega^{\rm ext})$, respectively.

The converse direction follows by repeating the same steps in the opposite direction.
\end{proof}

In order to prove Estimates~\eqref{eq:New_2_ext} and \eqref{eq:New_2_int}, we will make use of the Poisson integral representation of harmonic functions on an infinite strip. We thus recall in the next subsection some basic properties of the Poisson kernel on the strip.

\subsection{Poisson kernel on the infinite strip}

It is well known that (well-behaved) harmonic functions in an infinite strip in $\mathbb{R}^2$ can be represented as a convolution of appropriate boundary data with the Poisson kernel. For the sake of coherent exposition, we now recall this result and some related notions.


\begin{definition}[Poisson kernel on the infinite strip]\label{def:Poisson_strip} The Poisson kernel on the infinite strip $\mathcal{S}_0:= \R \times (0,\pi)$ is the function $\mathscr{P} \colon \mathcal{S}_0 \rightarrow \mathbb{R}$ given by
	\begin{align}
	\forall (\tau,\theta) \in \mathcal{S}_0\colon \quad	\mathscr{P}(\tau,\theta) = \mathscr{P}_\theta(\tau) := \frac{1}{2\pi}  \frac{\sin(\theta) }{\cosh(\tau)- \cos(\theta)}. \label{eq:Poissondef}
		\end{align}
	\end{definition}

We then have the following representation for harmonic functions on the strip $\mathcal{S}_0$.

\begin{lemma}[Poisson integral on the strip \cite{widder1961functions}]\label{lem:Widder} Let $\mathcal{S}_0:= \mathbb{R} \times (0, \pi)$ be the the infinite strip, let $\mathscr{P}\colon \mathcal{S}_0 \rightarrow \R$ be the Poisson kernel defined in Equation~\eqref{eq:Poissondef}, and for any $g,h \in C_c^\infty(\R)$, let $u_{g,h}\colon  \mathcal{S}_0 \rightarrow \R$ be the function defined as
	\begin{align}
	\forall (\tau,\theta)\in \mathcal{S}_0 \colon\quad  	u_{g,h}(\tau,\theta) := \int_{-\infty}^{\infty} \mathscr{P}_\theta(\tau - \xi)g(\xi)\, d\xi+  \int_{-\infty}^{\infty} \mathscr{P}_{\pi- \theta}(\tau-\xi)h(\xi)\, d\xi. \label{eq:poissonintegralstrip}
		\end{align}
	Then $u_{g,h}$ is the unique bounded harmonic function in $\mathcal{S}_0$ satisfying $u_{g,h}(\cdot,\theta) \rightarrow g $ and $u_{g,h}(\cdot,\theta) \rightarrow h$ uniformly as $\theta \rightarrow 0$ and $\theta \ra \pi$, respectively. 
	\end{lemma}

\begin{proof}
The proof of the above lemma is rather standard and relies on the fact that the Poisson kernel is an approximation of the identity; the uniqueness follows from the classical $L^\infty$ maximum principle. We shall, therefore, omit the details and refer to \cite{widder1961functions}, where a detailed study of the Poisson kernel on the strip is carried out.
\end{proof}

As a consequence of Lemma~\ref{lem:Widder}, we can show that the pull-back of the Poisson integral on the disk $ \Psi(\mathcal{S}_\sigma)$ for $\sigma \in (0,\pi)$ is the Poisson integral on the strip $\mathcal{S}_\sigma = \R \times (\sigma,\sigma+\pi)$ defined via~\eqref{eq:poissonintegralstrip}. This fact, or more generally, the fact that the Poisson integral on different domains is preserved under the pull-back of conformal transformations is well-known. Nevertheless, we provide a proof for the sake of completeness.

\begin{lemma}[Pull-back of the Poisson integral]\label{lem:Poissonintegralstrip} Let $\Psi \colon \mathcal{S} \rightarrow \mathbb{R}^2$ be the bipolar transform given by Equation~\eqref{eq:bipolardef}, let  $\sigma \in (0,\pi)$ and $\mathcal{S}_{\sigma}:= \R \times (\sigma, \sigma+\pi)$ so that $\Psi(\mathcal{S}_{\sigma})$ is some open disk with radius $r_{\sigma}>0$ and center $\mathbf{x}_{\sigma} \in \mathbb{R}^2$. Moreover, for $f\in \mL^2\bigr(\partial \Psi(S_\sigma)\bigr)$ we let $u_f$ be the Poisson integral on the disk $\Psi(\mathcal{S}_\sigma)$,%\in \mH^{\frac{1}{2}}(\Psi(\mathcal{S}_{\sigma}))$ be the harmonic extension of $f$ defined through the Poisson integral formula 
\begin{align*}
\forall \mathbf{x} \in \Psi(\mathcal{S}_{\sigma}) \colon\quad  u_f(\mathbf{x}) \coloneqq \frac{1}{2\pi} \int_{\partial \Psi(\mathcal{S}_\sigma)} \frac{r_\sigma^2 - |\mathbf{x}-\mathbf{x}_\sigma|^2}{r_\sigma |\mathbf{x}-\mathbf{y}|^2} f(\mathbf{y}) \mathrm{d} \mathcal{H}^1(\mathbf{y}).
\end{align*}
Then the pull-back $\Psi_\# u_f := u_f \circ \Psi \rvert_{\mathcal{S}_\sigma}$ satisfies
\begin{align}
\forall (\tau,\sigma+\theta) \in \mathcal{S}_\sigma \colon \quad	(\Psi_\# u_f)(\tau, \sigma+\theta) =  \int_\R \mathscr{P}_{\theta}(\tau-\xi) g(\xi) \mathrm{d} \xi + \int_\R \mathscr{P}_{\pi-\theta}(\tau-\xi) h(\xi) \mathrm{d} \xi, \label{eq:Poissonintegralstrip2}
\end{align}
where $g$ and $h$ are the pull-back of the boundary data $f$ restricted to $\Psi(\R_\sigma)$ and $\Psi(\R_{\sigma+\pi})$, i.e., %f \rvert_{\Psi(\R_\sigma)}$ and $f \rvert_{\Psi(\R_{\sigma+\pi})}$, respectively}
\begin{align*}
    g(\xi) \coloneqq (\Psi_\# f\rvert_{\Psi(\R_{\sigma})})(\xi) = f \bigr(\Psi(\xi,\sigma)\bigr) \quad \text{and} \quad
    h(\xi) \coloneqq (\Psi_\# f \rvert_{\Psi(\R_{\sigma+\pi})})(\xi) = f \bigr(\Psi(\xi,\sigma+\pi)\bigr),
\end{align*}
and we recall the notation, $\R_{\delta}:= \R \times \{\delta\}$ for all $\delta \in \mathbb{R}$.
\end{lemma}
\begin{proof} 
Since $\partial \Psi(\mathcal{S}_\sigma) \setminus \bigr(\Psi(\R_\sigma) \cup \Psi(\R_{\sigma+\pi})\bigr) = \{ \mathbf{a}_1,\mathbf{a}_2\}$ has zero $\mathcal{H}^1$ measure, we deduce that 
\begin{align}
	(\Psi_\# u_f)(\tau,\sigma+\theta) &= \frac{1}{2\pi} \int_{\Psi(\R_\sigma)} \frac{r_\sigma^2 - |\mathbf{x}-\mathbf{x}_\sigma|^2}{r_\sigma |\mathbf{x}-\by|^2} f(y) \mathrm{d} \mathcal{H}^1(\by) + \frac{1}{2\pi} \int_{\Psi(\R_{\sigma+\pi})} \frac{r_\sigma^2 - |\bx-\bx_\sigma|^2}{r_\sigma |\bx-\by|^2} f(y) \mathrm{d} \mathcal{H}^1(\by) \nonumber \\
	&= \int_\R T_1(\tau,\xi,\sigma,\theta) g(\xi) \mathrm{d} \xi + \int_\R T_2(\tau,\xi,\sigma,\theta) h(\xi) \mathrm{d} \xi, \label{eq:intermediate}
\end{align}
holds for all $(\tau,\sigma+\theta) \in \mathcal{S}_\sigma$ and for some suitable smooth functions $T_1$ and $T_2$. Hence, it is enough to show that for all $\tau,\xi \in \R$ and all $\sigma,\theta \in (0,\pi)$, it holds that
\begin{align}
	T_1(\tau,\xi,\sigma,\theta) = \mathscr{P}_\theta(\tau-\xi)\quad \mbox{and}\quad T_2(\tau,\xi,\sigma,\theta) = \mathscr{P}_{\pi-\theta}(\tau-\xi). \label{eq:funid}
\end{align}


To this end, it suffices to consider functions $f \in C_c^\infty\bigr(\Psi(\R_\sigma) \cup \Psi(\R_{\sigma+\pi})\bigr)$. Indeed, if the right hand side of \eqref{eq:intermediate} is equal to \eqref{eq:Poissonintegralstrip2} for every $f \in C_c^\infty\bigr(\Psi(\R_\sigma) \cup \Psi(\R_{\sigma+\pi})\bigr)$, then \eqref{eq:funid} holds by a density argument. We can now finish the proof by noticing that, for $f \in C_c^\infty\bigr(\Psi(\R_\sigma) \cup \Psi(\R_{\sigma+\pi})\bigr)$, the pull-back $\Psi_\# u_f$ is continuous and bounded up to the boundary of $\mathcal{S}_\sigma$, and therefore, the right-hand side of \eqref{eq:intermediate} must agree with \eqref{eq:Poissonintegralstrip2} by the uniqueness of the Poisson integral representation on the strip $\mathcal{S}_0$ given in Lemma~\ref{lem:Widder}.
\end{proof}

Lemma~\ref{lem:Poissonintegralstrip} together with the prior Lemma \ref{lem:L2maxstrip} allows us to restate the original Theorem~\ref{thm:main}-- which involved harmonic functions on a disk-- in terms of boundedness properties of the Poisson integral on the strip with respect to the weighted Lebesgue spaces $\mathcal{L}^2_\sigma$. More precisely, let us define the harmonic extension operator at height $\theta \in (0, \pi)$ as the mapping $P_\theta\colon \mathcal{L}^2_{\sigma} \rightarrow C^\infty(\R)$ given by
\begin{align}
\forall	g\in \mathcal{L}^2_{\sigma}, \forall \tau \in \mathbb{R}\colon \quad (P_\theta g)(\tau) = \int_\R \mathscr{P}_\theta(\tau-\xi) g(\xi) \mathrm{d} \xi. \label{eq:Pdef}
\end{align}
We then have the following reformulation of Theorem~\ref{thm:main}.

\begin{lemma}[Weighted $\mL^2$ estimates %-maximum principle
for the Poisson kernel]\label{lem:L2maxpoisson} Consider the alternative definition of the weighted Lebesgue spaces $\mathcal{L}^2_\sigma$ given by Remark \ref{def:Leb_w_2} and %for any $\theta \in (0, \pi)$
let $P_\theta\colon \mathcal{L}^2_{\sigma} \rightarrow C^\infty(\R)$ be the harmonic extension operator at height $\theta$ %be
defined through Equation~\eqref{eq:Pdef}. Then Estimates~\eqref{eq:New_2_ext} and \eqref{eq:New_2_int} %~\eqref{eq:New_2_ext}--\eqref{eq:New_2_full} 
hold if and only if
\begin{align}
	\norm{P_\theta g}_{\mathcal{L}^2_{\sigma+\theta}}^2 < \frac{1+\cos(\theta)}{2} \norm{g}_{\mathcal{L}^2_{\sigma}}^2,\label{eq:New_3}
\end{align}
for all $g \in \mathcal{L}^2_{\sigma}$ and any $\sigma,\theta \in (0,\pi)$. Moreover, Estimates~\eqref{eq:New_2_ext} and \eqref{eq:New_2_int} %~\eqref{eq:New_2_ext}--\eqref{eq:New_2_full}
are sharp if and only if 
\begin{align}
	\norm{P_\theta}_{\mathcal{L}^2_\sigma \rightarrow \mathcal{L}^2_{\sigma+\theta}}^2 \coloneqq \sup_{g \in \mathcal{L}^2_{\sigma}\setminus \{0\}} \frac{\norm{P_\theta g}_{\mathcal{L}^2_{\sigma+\theta}}^2}{\norm{g}_{\mathcal{L}^2_\sigma}^2} = \frac{1+\cos(\theta)}{2} \quad %\mbox{and}\quad \sup_{(g,h) \in \mathcal{L}^2_\sigma\oplus \mathcal{L}^2_{\sigma+\pi}\setminus \{0\}} \frac{\norm{P_\theta g + P_{\pi-\theta} h}_{\mathcal{L}^2_{\sigma+\theta}}^2}{\norm{g}_{\mathcal{L}^2_\sigma}^2 + \norm{h}_{\mathcal{L}^2_{\sigma+\pi}}^2} = 1,
\end{align}
for any $\sigma,\theta \in (0,\pi)$.
\end{lemma}

\begin{proof} From the Poisson integral representation formula in~\eqref{eq:Poissonintegralstrip2}, it is clear that Estimate \eqref{eq:New_3} is equivalent to Estimate \eqref{eq:New_2_ext}. To see that \eqref{eq:New_3} is also equivalent to Estimate \eqref{eq:New_2_int}, we note that for any $\theta, \sigma \in (0, \pi)$ and all measurable functions $g\colon \R \rightarrow \R$ we have 
\begin{align*}
	\norm{g}_{\mathcal{L}^2_{\sigma+\theta}} = \norm{g}_{\mathcal{L}^2_{2\pi-\sigma-\theta}}\quad \mbox{and}\quad \norm{g}_{\mathcal{L}^2_{\sigma+\pi}} = \norm{g}_{\mathcal{L}^2_{\pi-\sigma}}.
\end{align*}
Indeed, this is simply a consequence of the fact that the cosine function is even and $2\pi\imath$ periodic. In particular $\cos(\pi+\theta) = -\cos(\theta)$, and we also have%and we find that Estimate \eqref{eq:New_2_int} is equivalent to 
\begin{align*}
\norm{P_{\pi-\theta_{\Omega}} g}_{\mathcal{L}^2_{\theta_{\Omega}+\sigma}}^2=\norm{P_{\pi-\theta} g}_{\mathcal{L}^2_{2\pi-\theta-\sigma}}^2 \quad &\text{and} \quad \frac{1-\cos(\theta)}{2} \norm{g}_{\mathcal{L}^2_{\sigma+\pi}}^2=\frac{1+\cos(\pi-\theta)}{2} \norm{g}_{\mathcal{L}^2_{\pi-\sigma}}^2\\
\intertext{so that}
\norm{P_{\pi-\theta} g}_{\mathcal{L}^2_{\theta+\sigma}}^2 < \frac{1-\cos(\theta)}{2} \norm{g}_{\mathcal{L}^2_{\sigma+\pi}}^2 &\iff \norm{P_{\pi-\theta} g}_{\mathcal{L}^2_{2\pi-\theta-\sigma}}^2 < \frac{1+\cos(\pi-\theta)}{2} \norm{g}_{\mathcal{L}^2_{\pi-\sigma}}^2.
\end{align*}
Lemma \ref{lem:Poissonintegralstrip} implies that the inequality appearing on the left-hand side above is precisely Estimate \eqref{eq:New_2_int} while the inequality appearing on the right-hand side above is precisely Estimate~\eqref{eq:New_3} with $\theta,\sigma$ replaced by $\pi-\theta$ and $\pi-\sigma$. %Next, we claim that Equation~\eqref{eq:New_2_full} follows from \eqref{eq:New_3}. Indeed, recalling once again Lemma~\ref{lem:Poissonintegralstrip} and using the Cauchy-Schwarz inequality, we deduce that for all $\theta, \sigma \in (0, \pi)$, all $g \in \mathcal{L}^2_{\sigma}$ and all $h \in \mathcal{L}^2_{\sigma+\pi}$ it holds that
%\begin{align*}
	%\norm{\big((u_g + u_h)\circ \Psi\big)(\cdot,\sigma+\theta)}_{\mathcal{L}^2_{\sigma+\theta}}^2 &< \norm{P_\theta g}_{\mathcal{L}^2_{\sigma+\theta}}^2 + \norm{P_{\pi-\theta} h}_{\mathcal{L}^2_{\sigma+\theta}}^2 + 2 \norm{P_\theta g}_{\mathcal{L}^2_{\sigma+\theta}} \norm{P_{\pi-\theta} g}_{\mathcal{L}^2_{\sigma+\theta}} \\
	%&\leq \frac{1+\cos(\theta)}{2} \norm{g}_{\mathcal{L}^2_\sigma}^2 + \frac{1-\cos(\theta)}{2} \norm{h}_{\mathcal{L}^2_{\sigma+\pi}}^2 \\
% &\ \ + \sqrt{1-\cos(\theta)^2} \norm{g}_{\mathcal{L}^2_{\sigma}} \norm{h}_{\mathcal{L}^2_{\sigma+\pi}} \\
%	& \leq \norm{g}_{\mathcal{L}^2_{\sigma}}^2 + \norm{h}_{\mathcal{L}^2_{\sigma+\pi}}^2.
%\end{align*}
Since the sharpness statement is immediate, this completes the proof.
\end{proof}

\textcolor{orange}{\begin{remark}[Weighted $\mL^p$ estimates for Poisson kernel] \label{rem:Lpests} We can also use Lemma~\ref{lem:L2maxstrip} and the Poisson integral representation \eqref{eq:Poissonintegralstrip2} to re-state the $\mL^p$ estimates in Corollary~\ref{cor:Lpest} in terms of the operator norm of $P_\theta$ with respect to the weighted Lebesgue spaces $\mathcal{L}^p_{\sigma}$. In particular, estimates~\eqref{eq:Linf_int} and \eqref{eq:Linf_ext} from \cite{ciaramella2018analysis} are equivalent to
\begin{align}
    \norm{P_\theta}_{\mL^\infty(\R) \rightarrow \mL^\infty(\R)} \leq \frac{\pi-\theta}{\pi}, \quad \mbox{for any $\theta \in (0,\pi)$.} \label{eq:Linfnorm}
\end{align}
Note that, since the Poisson kernel $\mathscr{P}_\theta$ is positive, the above operator norm is given by the integral $\int_{\R} \mathscr{P}_\theta(\tau) \mathrm{d} \tau$. Consequently, estimate~\eqref{eq:Linfnorm} follows from %that $\int_\R \mathscr{P}_\theta(\tau) \mathrm{d} \tau = \frac{\pi-\theta}{\pi}$ (see 
Corollary~\ref{cor:PoissonFourier} below.
\end{remark}}

\textcolor{orange}{\begin{remark*}[Sharpness of $\mL^2$ maximum principle for circular arcs across $\Omega$] \label{rem:sharpest} Similarly, one can show that estimate~\eqref{eq:New_1_full} is sharp if and only if
\begin{align}
    \sup_{g \in \mathcal{L}^2_\sigma , h \in \mathcal{L}^2_{\sigma+\pi}} \frac{\norm{P_\theta g + P_{\pi-\theta} h}_{\mathcal{L}^2_{\sigma+\theta}}^2}{\norm{g}_{\mathcal{L}^2_\sigma}^2 + \norm{h}_{\mathcal{L}^2_{\sigma+\pi}}^2} = 1. \label{eq:sharpest2}
\end{align}
This estimate can be proved via the methods used in Section~\ref{sec:mainproofs} (see Remark~\ref{rem:sharpest2})
\end{remark*}}




==> concentric_circle.tex <==
\begin{figure}[t!]
\begin{center}
\begin{tikzpicture}[scale=1.0]
%Draw Axis
%\draw[<->,line width=0.6pt] (-3,0)--(3,0) node[right]{$x$};
%\draw[<->,line width=0.6pt] (0,-3)--(0,3) node[right]{$y$};

%Center circle
\draw[line width=1pt] (0,0) circle [radius=2];
\draw[line width=1pt, crimson] (0,0) circle [radius=1.4];
%Cocentric dotted circles
\draw[line width=0.8pt, crimson, dashdotted] (0,0) circle [radius=1.05];
%\draw[line width=0.8pt, crimson, dashdotted] (0,0) circle [radius=0.75];
\draw[line width=0.8pt, crimson, dashdotted] (0,0) circle [radius=0.7];
\draw[line width=0.8pt, crimson, dashdotted] (0,0) circle [radius=0.35];

\draw[line width=0.8pt, blue] (0,-0.4) circle [radius=1];

%Radii lines
\draw[line width=0.8pt, dotted] (0,0)--(-2	,0); 
\draw[line width=0.8pt, dotted] (0,0)--(0,1.4); 

%Draw bullet points in the center of circle
\filldraw[line width=0.8pt] (0,0) circle [radius=0.05];
\begin{scriptsize}
\draw (-1.6,0.75) node[align=center] {\small{$\Omega$}};
\draw (0.45,-1.1) node[align=center] {\small{$\textcolor{blue}{\Gamma}$}};
\draw (-1.6,0.15) node[align=center] {\small{$r_{\Omega}$}};
\draw (0.24,0.85) node[align=center] {\small{$r_{\Gamma}$}};
\draw (0.1,-0.24) node[align=center] {\small{$\mathbf{x}_{\Omega}$}};
\end{scriptsize}
\end{tikzpicture}
\caption{2-D schematic diagram of family of concentric circles approximating the smallest circle that is concentric to $\partial \Omega$ and contains the maximal arc $\Gamma$.}\label{fig:concentric}
\end{center}
\end{figure}
